Adaptive Rule Discovery for Labeling Text Data

Creating and collecting labeled data is one of the major bottlenecks in machine learning pipelines and the emergence of automated feature generation techniques such as deep learning, which typically requires a lot of training data, has further exacerbated the problem. While weak-supervision techniques have circumvented this bottleneck, existing frameworks either require users to write a set of diverse, high-quality rules to label data (e.g., Snorkel), or require a labeled subset of the data to automatically mine rules (e.g., Snuba). The process of manually writing rules can be tedious and time consuming. At the same time, creating a labeled subset of the data can be costly and even infeasible in imbalanced settings. This is due to the fact that a random sample in imbalanced settings often contains only a few positive instances. To address these shortcomings, we present Darwin, an interactive system designed to alleviate the task of writing rules for labeling text data in weakly-supervised settings. Given an initial labeling rule, Darwin automatically generates a set of candidate rules for the labeling task at hand, and utilizes the annotator's feedback to adapt the candidate rules. We describe how Darwin is scalable and versatile. It can operate over large text corpora (i.e., more than 1 million sentences) and supports a wide range of labeling functions (i.e., any function that can be specified using a context free grammar). Finally, we demonstrate with a suite of experiments over five real-world datasets that Darwin enables annotators to generate weakly-supervised labels efficiently and with a small cost. In fact, our experiments show that rules discovered by Darwin on average identify 40% more positive instances compared to Snuba even when it is provided with 1000 labeled instances.

==> build_sketch.tex <==
Given a sentence $s$ and a grammar $\mathcal{G}$, we can generate an operator sketch for $s$ very quickly. One simple way to generate the operator sketch is to consider all possible applications of the operators to generate a sentence and then represent them in the form of a hierarchy, merging any duplicate operators at the same level. It is a compact representation of all the operators of the grammar that can generate the sentence. The operator sketch is generated by basic operators only. Any operator which can be imitated by multiple applications of some other operator is not considered as a basic operator. eg. Consider a grammar of tree queries, with two different operators: descendants and children. The descendant operator can be seen as a generalization of the child. Hence, the operator sketch will be built using children queries and not the descendants. 

Operator sketch is a powerful representation of the grammar in the form of a hierarchy for a particular instance of the corpus. Notice that 
With small changes in the grammar, the operator sketch can be modified accordingly eg. Consider the modified multigram grammar where consecutive tokens in the rule can have maximum of any two tokens between them. In such a case, we can use the operator sketch from multigram grammar and add more edges eg. 'what-the' and 'what-best' are two new edges added. 
For simplicity, it is better to assume each node in operator sketch has an inverted list with a single element pointing to the sentence for which the sketch is generated.

==> tree_grammar.tex <==
Here, we demonstrate the behavior of Darwin given a more complex rule grammar. This
grammar generates rules over the dependency parse trees of sentences. Such rules
over the dependency structure are commonly used in information extraction
tasks~\cite{Odin, koko} to capture the semantic relationships between the tokens in
the sentence. The grammar we consider, called TreeMatch, is the following:

\smallskip
\noindent\textbf{Terminals} (denoted by $V$): All tokens and Part-of-Speech
(POS) tags~\cite{pos} present in the corpus. E.g., NOUN, VERB, etc.

\noindent\textbf{Derivation Rules:} The grammar has three fundamental symbols
that make up a rule, namely And ($\wedge$), Child (/), and Descendant (//). 
%\wctan{btw, we should clarify what an ``operator'' meant in the PhraseMatch grammar. the word operator came out of the blue in section 3.}
The symbol `a/b' implies that terminal `b' should be a child of terminal `a' in
the dependency parse tree. The symbol `a//b' implies that terminal `b' should be
a descendant of terminal 'a' in the parse tree. Given that, the derivation rules of
the grammar are:
\begin{alltt}
    A \(\rightarrow\) /A
    A \(\rightarrow\) A\(\wedge\)A
    A \(\rightarrow\) //A
    A \(\rightarrow\) v (\(\forall v\in\mathcal{V}\))
\end{alltt}
\begin{figure}[b]
\includegraphics[scale=0.25]{kokosentence.pdf}
\caption{An example of a parse tree\label{fig:tree_grammar}.}
\vspace{-.4em}
\end{figure}

An example rule for this grammar is `//way/ADJ$\,\wedge\,$to//NOUN'. This rule
considers all sentences which have `way' as any descendant of the root of the
dependency tree, an adjective and the word `to' as children of the token `way',
and a NOUN as a descendant of the token `to'. Figure~\ref{fig:tree_grammar}
shows the parse tree of a sentence that satisfies this rule.

Clearly, the TreeMatch grammar is more complex compared to the PhraseMatch grammar as it
looks into the dependency trees of sentences. In fact, given that PhraseMatch
rules require the words to appear consequently, there are only $t(t+1)/2$ rules
matching a sentence with $t$ tokens. However, this constraint is absent from
the TreeMatch, therefore there are at least $2^{t+1}$ rules that simply enforce 
which subset of the words should be present in the sentence.

\noindent\textbf{Derivation Sketch:} 
%Even though the tree based grammar can
%generate many complex rules, 
%The operator sketch of a sentence is the dependency parse
%tree of the sentence. 
The derivation sketch can be created as explained by enumerating all sequence of
derivations up to a fixed number of steps. However, a more compact derivation sketch for
the TreeMatch grammar is simply the dependency parse tree of the sentence, as we can use
it to quickly check whether a rule matches the parse tree or not.
\iffalse
of a sentence is constructed using
the child operator and $\wedge$ operators alone. The descendant operator is
complex and we simulate the descendant operator by applying the child operator multiple
times. \wctan{w.r.t. the previous sentence, is it because we bound the expansion of the // operator? Or do we find all expansions w.r.t. a given sentence. That is, a sentence can have multiple parse trees depending on how you parse the descendant operator. I rephrased but I think it is still not clear.} 
\fi
Figure \ref{fig:tree_grammar} shows the dependency parse tree of a sentence which can serve as its derivation sketch as well.
Given the exponentially many candidate rules generated by this grammar, the candidate-rule
generation step is crucial for pruning useless rules to identify a smaller set of
candidates. We evaluate the performance of \darwin\ with this grammar in the
next section.
